Priced Timed Petri Nets

We consider priced timed Petri nets, i.e., unbounded Petri nets where each token carries a real-valued clock. Transition arcs are labeled with time intervals, which specify constraints on the ages of tokens. Furthermore, our cost model assigns token storage costs per time unit to places, and firing costs to transitions. This general model strictly subsumes both priced timed automata and unbounded priced Petri nets. We study the cost of computations that reach a given control-state. In general, a computation with minimal cost may not exist, due to strict inequalities in the time constraints. However, we show that the infimum of the costs to reach a given control-state is computable in the case where all place and transition costs are non-negative. On the other hand, if negative costs are allowed, then the question whether a given control-state is reachable with zero overall cost becomes undecidable. In fact, this negative result holds even in the simpler case of discrete time (i.e., integer-valued clocks).

==> translation.tex <==
\begin{lemma}\label{lem:automata_oracle}
Given a configuration-automaton $\automaton$,
$C$ as in Lemma~\ref{lem:AC-PTPN-reach},
and a finite set $U\subseteq \uc{C}$,
it is decidable if there exists some
AC-PTPN configuration 
$\initconf \in \wordencoding^{-1}(L(\automaton))$ s.t. $\initconf \rightarrow_A^* \uc{U}$.
\end{lemma}
\begin{proof}
The idea is to translate the AC-PTPN into an SD-TN which simulates its
computation. The automaton $\automaton$ is also encoded into the SD-TN and
runs in parallel. $\automaton$ outputs an encoding of $\initconf$, a nondeterministically
chosen initial AC-PTPN configuration from $L(\automaton)$.
Since the SD-TN cannot encode sequences, it cannot store the order information in
the sequences which are AC-PTPN configurations. Instead this is encoded into
the behavior of $\automaton$, which outputs parts of the configuration $\initconf$
`just-in-time' before they are used in the computation (with exceptions;
see below).
Several abstractions are used to unify groups of tokens with different
fractional parts, whenever the PTPN is unable to distinguish them.
AC-PTPN timed transitions of types 1 and 2 are encoded as SD-TN transfer
transitions, e.g., all tokens with integer age advance to an age with a small
fractional part. Since this operation must affect all tokens, it cannot
be done by ordinary Petri net transitions, but requires the
simultaneous-disjoint transfer of SD-TN. Another complication is that the
computation of the AC-PTPN might use tokens (with high fractional part) from
$\initconf$, which the automaton $\automaton$ has not yet produced.
This is handled by encoding a `debt' on future outputs of $\automaton$ in
special SD-TN places. These debts can later be `paid back' by outputs of
$\automaton$ (but not by tokens created during the computation).
At the end, the computation must reach an encoding of a configuration in
$\uc{U}$ and all debts must be paid. This yields a reduction to a reachability
problem for the constructed SD-TN, which is decidable by
Theorem~\ref{thm:SD-TN-reachability}.

We devote the rest of the section to give the details of the proof.
%

We show the lemma for the case where $U$ is a singleton
$\set{\finalconf}$.
%
The result follows from the fact that $U$ is finite and that
$\uc{U}=\cup_{\conf\in U}\uc{\conf}$.
%
We will define an SD-TN 
$\sdtn=\tuple{\states^{\sdtn},\places^{\sdtn},\transitions^{\sdtn},\transfer^{\sdtn}}$,
a finite set $\initsdtnconfs$ of (initial) configurations, 
and a finite set of (final) $\omega$-configurations $\finalsdtnconfs$ such that
$\exists\initsdtnconf\in\initsdtnconfs.\;
\exists\finalsdtnconf\in\finalsdtnconfs.\;
\initsdtnconf\movesto{*}\finalsdtnconf$ in $\sdtn$ iff
there is
a $\initconf \in \wordencoding^{-1}(L(\automaton))$ s.t. $\initconf \rightarrow_A^* \uc{U}$.
%
The result then follows immediately from Theorem~\ref{thm:SD-TN-reachability}
(and Corollary~\ref{cor:SD-TN-reachability}).
Let
$\finalconf=\tuple{\tuple{\state_{\it fin},y_{\it fin}},\finalmarking}$ where
$\finalmarking$ is of the form
$\tuple{\mset_{-m}\cdots\mset_{-1},\mset_0,\mset_1\cdots\mset_n}$ and
$\mset_i$ is of the form
$\tuple{\tuple{\place_{i1},k_{i1}},\ldots,\tuple{\place_{in_i},k_{in_i}}}$
for $i:-m\leq i\leq n$.
%
Let the finite-state automaton $\automaton$ be of the form 
$\tuple{\states^{\cal A},\transitions^{\cal A},\state^{\cal A}_0,\fstates^A}$
where $\states^{\cal A}$ is the set of states,
$\transitions^{\cal A}$ is the transition relation,
$\state^{\cal A}_0$ is the initial state, and
$\fstates^{\cal A}$ is the set of final states.
%
A transition in $\transitions^{\cal A}$ is of the form
$\tuple{\state_1,a,\state_2}$ where
$\state_1,\state_2\in\states^{\cal A}$ and 
$a\in\left(\places\times\zeroto{\maxval +1}\right)
\cup
(\states\times\setcomp{y}{0\leq v\leq y_{\it init}})
\cup
\set{\sep,\$}$.
%
We write $\state_1\movesto{a}\state_2$ to denote that
$\tuple{\state_1,a,\state_2}\in\transitions^{\cal A}$.
%
During the operation of $\sdtn$, we will run the automaton
$\automaton$ ``in parallel'' with $\tpn$.
%
%From time to time, we perform one step of $\automaton$.
%
During the course of the simulation, the automaton
$\automaton$ will generate the encoding of a configuration
$\initconf$.
%
We know that such an encoding consists of 
a control-state $\tuple{\initstate,y_{\it init}}$ followed by the
encoding of a  marking
$\initmarking$, say of the form
$\tuple{\cmset_{-m'}\cdots\cmset_{-1},\cmset_0,\cmset_1\cdots\cmset_{n'}}$.
%
Notice that $\automaton$ may output the encoding of any marking
in its language, and therefore the values of $m'$ and $n'$
are not a priori known.
                      



To simplify the presentation, we introduce a number of conventions for the description
of $\sdtn$.
%
First we define a set $\vars$ of variables (defined below), 
where each variable $\var\in\vars$ ranges over a finite domain $\domof{\var}$.
%
A control-state $\state$ then is a mapping that assigns, to each variable
$\var\in\vars$, a value in $\domof{\var}$, i.e., $\state(\var)\in\domof{\var}$.
%
Consider a state $\state$, variables $\var_1,\ldots,\var_n$ where $\var_i\neq\var_j$ if $i\neq j$,
and values $\val_1,\ldots,\val_n$ where $\val_i\in\domof{\var_i}$ for all $i:1\leq i\leq n$.
%
We use $\state[\var_1\assigned\val_1,\ldots,\var_k\assigned\val_k]$ to denote that
state $\state'$ such that $\state'(\var_i)=\val_i$ for all $i:1\leq i\leq k$,
and $\state'(\var)=\state(\var)$ if $\var\not\in\set{\var_1,\ldots,\var_k}$.
%
Furthermore, we introduce a set of \emph{transition generators}, where each
transition generator $\transgen$ characterizes a (finite) set $\denotationof{\transgen}$
of transitions in $\sdtn$.
%
A transition generator $\transgen$ is a tuple
$\tuple{\precondof{\transgen},
\postcondof{\transgen},\inputsof{\transgen},\outputsof{\transgen}}$,
where
\begin{itemize}
\item
$\precondof{\transgen}$ is a set 
$\set{\var_1=\val_1,\ldots,\var_k=\val_k}$,
where $\var_i\in\vars$ and $\val_i\in\domof{\var_i}$ for all $i:1\leq i\leq k$.
%
\item
$\postcondof{\transgen}$ is a set 
$\set{\var'_1\assigned\val'_1,\ldots,\var'_\ell\assigned\val'_\ell}$,
where $\var'_i\in\vars$ and $\val'_i\in\domof{\var'_i}$ for all $i:1\leq i\leq \ell$.
\item
$\inputsof{\transgen},\outputsof{\transgen}\in \msetsover{\left(\places^\sdtn\right)}$.
\end{itemize}
%
The set $\denotationof\transgen$ contains all transitions of the form
$\tuple{\state_1,\state_2,\inputs,\reads,\outputs}$ where
\begin{itemize}
\item
$\state_1(\var_i)=\val_i$ for all $i:1\leq i\leq k$.
\item
$\state_2=\state_1[\var'_1\assigned\val'_1,\ldots,\var'_\ell\assigned\val'_\ell]$.
\item
$\inputs=\inputsof{\transgen}$, and $\outputs=\outputsof{\transgen}$.
\end{itemize}
%
In the constructions we will define a set $\transgens$ of transition generators
and define $\transitions^\sdtn:=\cup_{\transgen\in\transgens}\denotationof\transgen$.
%

Below we will define the components
$\states^{\sdtn}$, $\places^{\sdtn}$, $\transitions^{\sdtn}$, and $\transfer^{\sdtn}$
in the definition of $\sdtn$, together with
the set $\initsdtnconfs$ and
configuration $\finalsdtnconf$.


\medskip
\noindent{\bf The set $\states^{\sdtn}$} is,
as mentioned above,  defined in terms of a set $\vars$ of variables.
%
The set $\vars$ contains the following elements:
\begin{itemize}
\item
$\mode$ indicates the \emph{mode} of the simulation.
%
More precisely, a computation of $\sdtn$ will consist of three phases, namely an
{\it initialization}, a {\it simulation}, and a {\it final phase}.
%
Each phase is divided into a number of sub-phases referred
to as {\it modes}.
%
\item
A variable $\nstate$, with $\domof{\nstate}=\states$, that
stores the current control-state $\state_\tpn$.
\item
A variable $\astate$, with $\domof{\astate}=\states_{\automaton}$, that
stores the current state of $\automaton$.
%
%
\item
A variable $\fstate{i,j}$ with $\domof{\fstate{i,j}}=\set{\true,\false}$,
for each $i:-m\leq i\leq n$ and $1\leq j \leq n_i$.
%
During the simulation phase, the systems tries to cover all the tokens
in the multisets of $\finalmarking$.
%
Intuitively, $\fstate{i,j}$ is a flag that indicates whether the token
$\tuple{\place_{i,j},k_{i,j}}$ has been covered.
%
\item
A variable $\coverflag$ that has one of the values $\on$ or $\off$.
%
The covering of tokens in $\finalmarking$ occurs only during certain phases 
of the simulation.
%
This is controlled by the value of the variable $\coverflag$.

\item
A variable $\coverindex$ with
$-m\leq\coverindex\leq n$ gives the next multiset whose tokens 
are to be covered.
\item
For each $\place\in\places$ and $k:0\leq k\leq\maxval+1$, we have a variable
$\rdebt{\place}{k}$, whose use and domain are explained below.
%
During the simulation, we will need to use tokens that
have still not been generated by $\automaton$.
%
To account for these tokens, we will implement a ``debt scheme''
in which tokens are used first, and then ``paid back'' by
tokens that are later generated by $\automaton$.
%
The variable $\rdebt{\place}{k}$ keeps track of the number of tokens
$\tuple{\place,k}$ that have been used on read arcs
(the debt on tokens consumed in input operations are managed
through specific places described later.)
%
For a place $\place$ and a transition $\transition$,
let $\maxread(\place,\transition)$ be the number of read arcs
between $\place$ and $\transition$.
%
Define $\maxread:=\max_{\place\in\places,\transition\in\transitions}\maxread(\place,\transition)$.
%
Then, $\domof{\rdebt{\place}{k}}=\set{0,\ldots,\maxread}$.
%
The  definition of the domain reflects the fact the largest amount of debt
that we will generate due to tokens raveling through read arcs is bounded by
$\maxread$.
\end{itemize}


\medskip
\noindent{\bf The set $\places^{\sdtn}$}
contains the following places:
\begin{itemize}
\item
For each 
$\place\in\places$ and $k:0\leq k\leq\maxval+1$, 
the set $\places^{\sdtn}$ contains the place
$\zeroplace{\place}{k}$.
%
The number of tokens in $\zeroplace{\place}{k}\in\places^{\sdtn}$ 
reflects (although it may be not exactly equal to)
the number of tokens
in $\place\in\places$ whose ages have zero fractional parts.
%
\item
For each 
$\place\in\places$ and $k:0\leq k\leq\maxval+1$, 
the set $\places^{\sdtn}$ contains the places
$\lowplace{\place}{k}$ and $\highplace{\place}{k}$.
%
These places play the same roles as above
for tokens with ages that have \emph{low} (close to $0$) resp. \emph{high}
(close to $1$) fractional parts.
%
\item
For each $\place\in\places$ and $0\leq k\leq\maxval+1$,
the set $\places^{\sdtn}$ contains the place
$\inputdebtplace{\place}{k}$.
%
The place represents the amount of debt due to tokens
$\tuple{\place,k}$ traveling through input arcs.
%
There is a priori no bound on the amount of debt on such tokens.
%
Hence, this amount is stored in places (rather than in variables
as is the case for read tokens.)
\end{itemize}

\medskip
\noindent{\bf The Set $\initsdtnconfs$}
contains all configurations $\tuple{\initstate^\sdtn,\initmarking^\sdtn}$
satisfying the following conditions:
\begin{itemize}
\item
$\initstate^\sdtn(\mode)=\initmode$.
%
The initial mode is $\initmode$.

\item
$\initstate^\sdtn(\astate)=\state^{\cal A}_0$.
%
The automaton $\automaton$
is simulated starting from its initial state $\state^{\cal A}_0$.
%
\item
$\initstate^\sdtn(\fstate{i,j})=\false$ 
for all $i:-m\leq i\leq n$ and $1\leq j \leq n_i$.
%
Initially we have not covered any tokens in $\finalmarking$.
\item
$\initstate^\sdtn(\rdebt{\place}{k})=0$
for all $\place\in\places$ and $k:0\leq k\leq\maxval+1$.
%
Initially, we do not have any debts due to read tokens.
\item
$\initmarking^\sdtn(\place)$ for all places $\place\in\places^\sdtn$.
%
Initially, all the places of $\sdtn$ are empty.
\end{itemize}
Notice that the variables $\coverflag$ and $\coverindex$ 
are not restricted so $\coverflag$ may be $\on$ or $\off$
and  $\coverindex$ may have any value $-m\leq\coverindex\leq n$.
%
Although $\nstate$ is not restricted either, 
its value will be defined in the first step of the simulation
(see below.)
%



Next, we explain how $\sdtn$ works.
%
In doing that, we also introduce all the members of the set $\transitions^\sdtn$.

\medskip
\noindent{\bf Initialization}
In the initialization phase
the SD-TN $\sdtn$ reads the initial control-state and then fills in the places according to $\initmarking$.
%
From the definition of the encoding of a configuration, we know that the automaton
$\automaton$ outputs a pair $\tuple{\state,y}$
 in its first transition.
%
The first move of $\sdtn$ is to store this pair in its control-state.
%
Thus, for each transition
$\state_1\movesto{\tuple{\state,y}}\state_2$ in $\automaton$ 
where $\state\in\states$ and $1\leq y \leq y_{\it init}$,
the set $\transgens$ contains $\transgen$ where:
%
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\initmode,\astate=\state_1}$.
\item
$\postcondof{\transgen}=\set{\mode\assigned\initlowmode,\nstate\assigned\tuple{\state,y},\astate\assigned\state_2}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\set{\lowplace{\place}{k}}$.
\end{itemize}
%
In other words, once $\sdtn$ has input the initial control-state, 
it enters a new mode $\initlowmode$.
%
In mode $\initlowmode$, we read the multisets
$\cmset_{1}\cdots\cmset_{m}$ that represent tokens with low fractional parts.
%
The system starts running $\automaton$ one step at a time, generating the elements
of $\cmset_m$ (that are provided by $\automaton$.)
%
When it has finished generating all the tokens in $\cmset_m$,
it moves to the next multiset, generating
the multisets one by one in the reverse order
finishing with $\cmset_{1}$.
%
We distinguish between two types of such tokens depending on
how they will be used in the construction.
%
More precisely, such a token is 
either {\it consumed} when firing transitions during the simulation phase
or  used for {\it covering} the multisets in $\finalmarking$.
%
A token (of the form $\tuple{\place,k}$), used for consumption,
is put in a place $\lowplace{\place}{k}$.
%
Recall that the relation $\amovesto{}$  in $\tpn$ is insensitive to the order of 
the fractional parts that are small (fractional parts of the tokens
in $\cmset_1,\ldots,\cmset_{n'}$.)
%
Therefore, tokens in  $\cmset_1,\ldots,\cmset_{n'}$
that have identical places $\place$ and identical integer parts $k$
will all be put in the same place $\lowplace{\place}{k}$.
%
Formally, for each transition
$\state_1\movesto{\tuple{\place,k}}\state_2$ in $\automaton$,
the set $\transgens$ contains $\transgen$ where:
%
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\initlowmode,\astate=\state_1}$.
\item
$\postcondof{\transgen}=\set{\astate\assigned\state_2}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\set{\lowplace{\place}{k}}$.
\end{itemize}
%
Each time a new multiset $\cmset_j$ is read from $\automaton$, 
the system decides whether 
it may be (partially) used for covering the next multiset $\mset_i$
in $\finalmarking$.
%
This decision is made by checking the value
of the component $\coverflag$.
%
if $\coverflag=\off$ then
the tokens are only used for consumption during the simulation phase.
%
However, if $\coverflag=\on$ then 
the tokens generated by $\automaton$ can also be used to cover those in $\finalmarking$.
%
The multiset currently covered is given by the value
of the component  $\coverindex$.
%
More precisely, if $\coverindex=i$ for some $i:1\leq i \leq n$ then
(part of) the multiset $\cmset_j$ that is
currently being generated by $\automaton$ ($j:1\leq j \leq n'$)
may be used to cover (part of) the multiset $\mset_i$.
%
At this stage, we only cover tokens with low fractional parts (those in the 
multisets $\mset_1,\ldots,\mset_n$.)
%
When using tokens for covering, the order on the fractional parts 
of tokens \emph{is} relevant.
%
The construction takes into consideration different aspects
of this order as follows:
\begin{itemize}
\item
According to the definition of the ordering $\lessfree$,
the tokens in a given multiset $\cmset_j$ 
may only be used to cover those in one and the same multiset (say $\mset_i$.)
%
This also agrees with the observation that
the tokens represented in $\cmset_j$ correspond to tokens in the original TPN 
that have identical fractional parts (the same applies to $\mset_i$.)
%
In fact, if this was not case, 
then we would be using tokens with identical fractional parts (in $\cmset_j$)
to cover tokens with different fractional parts.
%
Analogously, the multiset $\mset_i$ can be covered only by the elements
of one multiset $\cmset_j$.
%
\item
If $i'<i$ then the fractional parts of the tokens represented by 
$\mset_{i'}$ are smaller than those represented by $\mset_{i}$.
%
The same applies to $\cmset_{j'}$ and $\cmset_{j}$ if $j'<j$.
%
Therefore, if $\cmset_{j}$ is used to cover $\mset_{i}$ and $j'<j$ then
 $\cmset_{j'}$ should be used to cover $\mset_{i'}$ for some $i'<i$.
%
Furthermore, a multiset $\cmset_{j}$ is not necessarily used to 
cover any multiset, i.e.,
all the tokens represented by $\cmset_{j}$ 
may be used for consumption during the simulation
(none of them being used for covering.)
%
Similarly, it can be the case that a given  $\mset_{i}$ is not covered
by any multiset  $\cmset_{j}$ (all its tokens are covered by
tokens that are generated during the simulation.)
%
Also, a multiset $\cmset_{j}$ may only be partially used to cover
$\mset_{i}$, i.e., some of its tokens may be used for covering
$\mset_{i}$ while some are consumed during the simulation.
%
Finally,  $\mset_{i}$ may only be partially covered by $\cmset_{j}$, 
i.e., some of its tokens are
covered by $\cmset_{j}$ while the rest of tokens are covered by 
tokens generated during the simulation.
\end{itemize}
%
Formally, for each
$\state_1\movesto{\tuple{\place,k}}\state_2$ in $\automaton$,
$1\leq i\leq n$, $1\leq j\leq n_i$ with $\tuple{\place_{i,j},k_{i,j}}=\tuple{\place,k}$,
we add $\transgen$ to $\transgens$, where:
%
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\initlowmode,\astate=\state_1,$ $\coverflag=\on,\coverindex=i\}$.
\item
$\postcondof{\transgen}=\set{\astate\assigned\state_2,\fstate{i,j}\assigned\true}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
%
The transition sets the flag $\fstate{i,j}$ to $\true$ 
indicating that the token has now been covered.
%
A transition
$\state_1\movesto{\sep}\state_2$ in $\automaton$ indicates
that we have finished generating the elements of the current multiset $\cmset_j$.
%
If $\coverflag=\on$ then we have also finished covering tokens
in the multiset $\mset_i$.
%
Therefore, we decide the next multiset $i'<i$ in which which to cover tokens.
%
Recall that not all multisets have to be covered and 
hence $i'$ need not be equal to
$i-1$ (in fact the multisets $\mset_{i''}$ for $i'<i''<i$ 
will not be covered by the multisets in $\initmarking$.)
%
We also decide whether to use  $\initmset_{j-1}$ to cover  $\mset_{i'}$ or not.
%
In the former case, we set $\coverflag$ to $\on$, 
while in the latter case we
 set $\coverflag$ equal to $\off$.
%
Also, if $\coverflag=\off $ then we decide whether to use
$\cmset_{j-1}$ for covering
$\mset_{i}$ or not.
%
We cover these four possibilities by adding the following transition generators to $\transgens$.
%

(i) For each transition
$\state_1\movesto{\sep}\state_2$ in $\automaton$,
$i:1\leq i\leq n$, and $i':-m\leq i'<i$,
we add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\initlowmode,\astate=\state_1,\coverflag=\on,\coverindex=i\}$.
\item
$\postcondof{\transgen}=\{\astate\assigned\state_2,\coverindex\assigned i'\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
This is the case where $\coverflag$ is $\on$ and continues to be $\on$.
%
Notice that no covering takes place if $\coverindex\leq 0$,
and that the new value of $\coverindex$ is made strictly smaller than the current one.

(ii)
For each transition
$\state_1\movesto{\sep}\state_2$ in $\automaton$,
and each $i,i':1\leq i'<i\leq n$,
we add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\initlowmode,\astate=\state_1,$ 
$\coverflag=\on,\coverindex=i\}$.
\item
$\postcondof{\transgen}=\{\astate\assigned\state_2,\coverflag\assigned\off,\coverindex\assigned i'\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
This is the case where $\coverflag$ is $\on$ but it is turned $\off$
for the next step.
%

(iii)
For each transition
$\state_1\movesto{\sep}\state_2$ in $\automaton$,
we add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\initlowmode,\astate=\state_1,$ 
$\coverflag=\off\}$.
\item
$\postcondof{\transgen}=\{\astate\assigned\state_2\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
This is the case where $\coverflag$ is $\off$ and continues to be $\off$.

(iv) 
For each transition
$\state_1\movesto{\sep}\state_2$ in $\automaton$,
we add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\initlowmode,\astate=\state_1,$ 
$\coverflag=\off\}$.
\item
$\postcondof{\transgen}=\{\astate\assigned\state_2,\coverflag\assigned\on\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
%
This is the case where $\coverflag$ is $\off$ but it is turned $\on$
for the next step.
%



The process of generating tokens with low fractional parts
continues until we encounter a transition of the form
$\state_1\movesto{\$}\state_2$ in $\automaton$.
%
According to the encoding of markings, this indicates 
that we have finished generating the elements of the multisets $\cmset_1,\ldots,\cmset_n$.
%
Therefore, we change mode from $\initlowmode$ to
$\initzeromode$ (where we scan the multiset $\mset_0$.)
%
We have also to consider changing
the variables $\coverflag$ and $\coverindex$ in the 
same way as above.
%
Therefore, we add the following transition generators:

(i) 
For each transition $\state_1\movesto{\$}\state_2$ in $\automaton$,
$i:1\leq i\leq n$, and $i':-m\leq i'<i$,
we add $\transgen$ where:
%
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\initlowmode,\astate=\state_1,$ 
$\coverflag=\on,\coverindex=i\}$.
\item
$\postcondof{\transgen}=\{\mode\assigned\initzeromode,\astate\assigned\state_2,\coverflag\assigned\off,\coverindex\assigned i'\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}


(ii) 
For each transition $\state_1\movesto{\$}\state_2$ in $\automaton$,
$i:1\leq i\leq n$, and $i':-m\leq i'<i$,
we add $\transgen$ where:
%
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\initlowmode,\astate=\state_1,$ 
$\coverflag=\on,\coverindex=i\}$.
\item
$\postcondof{\transgen}=\{\mode\assigned\initzeromode,\astate\assigned\state_2,\coverflag\assigned\on,\coverindex\assigned i'\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}

(iii)
For each transition
$\state_1\movesto{\$}\state_2$ in $\automaton$,
we add $\transgen$ where:

\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\initlowmode,\astate=\state_1,$ 
$\coverflag=\off\}$.
\item
$\postcondof{\transgen}=\set{\mode\assigned\initzeromode,\astate\assigned\state_2}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}

(iv)
For each transition
$\state_1\movesto{\$}\state_2$ in $\automaton$,
we add $\transgen$ where:

\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\initlowmode,\astate=\state_1,$ 
$\coverflag=\off\}$.
\item
$\postcondof{\transgen}=\{\mode\assigned\initzeromode,\astate\assigned\state_2,\coverflag\assigned\on\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
%



In $\initzeromode$ the places are filled according to $\cmset_0$.
%
The construction is similar to the previous mode.
%
The only differences are that the tokens to be consumed will
be put in places $\zeroplace{\place}{k}$ 
and that no tokens are covered in $\finalmarking$.
%

For each transition
$\state_1\movesto{\tuple{\place,k}}\state_2$ in $\automaton$,
the set $\transgens$ contains $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\initzeromode,\astate=\state_1}$.
\item
$\postcondof{\transgen}=\set{\astate\assigned\state_2}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\set{\zeroplace{\place}{k}}$.
\end{itemize}
%
Since the tokens are not used at this stage
for covering the multisets of $\finalmarking$,
no transition generators are added for that purpose.
%
Also, in contrast to tokens belonging to 
$\cmset_0,\ldots,\cmset_{n'}$
we cannot generate tokens 
belonging to $\cmset_{-m'},\ldots,\cmset_{-1}$
during the initialization phase.
%
The reason is that, in the former case,
we only need to keep track of the order of multisets whose tokens are used for covering
(the ordering of the fractional parts in tokens used for consumption is not relevant.)
%
Since the number $n$ is given a priori in the construction (the marking
$\finalmarking$ is a parameter of the problem), we need only to keep track
of tokens belonging to at most $n$ different multisets.
%
This does not hold in the case of the latter tokens, 
since the order of the multisets to which the tokens belong is
relevant also in the case of tokens that will be consumed.
%
Since $m'$ 
is not a priori bounded, we postpone the generation of 
these tokens to the simulation phase, where we generate these tokens from
$\automaton$ ``on demand'': 
each time we perform a timed transition, we allow the 
$\highplace{\place}{k}$ tokens with the highest 
fractional part to be generated.
%
This construction is made more 
precise in the description of the simulation phase.
%
%

The mode $\initzeromode$ is concluded when we the next transition of 
$\automaton$ is labeled with $\$$.
%
This means that we have finished inputting the last multiset
$\mset_0$.
%
We now move on to the simulation phase.
%

For each transition of the form
$\state_1\movesto{\$}\state_2$ in $\automaton$, we add
$\transgen$ to $\transgens$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\initzeromode,\astate=\state_1}$.
\item
$\postcondof{\transgen}=\set{\mode\assigned\simmode,\astate\assigned\state_2}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}



\medskip
\noindent{\bf Simulation.}
The simulation phase consists of simulating a sequence of
transitions, each of which is either discrete, of type $1$, or of type $2$.
%
Each type $2$ transition is preceded by at least one type $1$ transition.
%
Therefore, from $\simmode$ we next perform a discrete or a type $1$  transition.
%
The (non-deterministic) choice is made
using the transition generators $\transgen_1$ and $\transgen_2$ 
where:
\begin{itemize}
\item
$\precondof{\transgen_1}=\set{\mode=\simmode}$.
\item
$\postcondof{\transgen_1}=\set{\mode\assigned\discmode}$.
\item
$\inputsof{\transgen_1}=\emptyset$.
\item
$\outputsof{\transgen_1}=\emptyset$.
\end{itemize}
\begin{itemize}
\item
$\precondof{\transgen_2}=\set{\mode=\simmode}$.
\item
$\postcondof{\transgen_2}=\set{\mode\assigned\typeoneamode}$.
\item
$\inputsof{\transgen_2}=\emptyset$.
\item
$\outputsof{\transgen_2}=\emptyset$.
\end{itemize}



\medskip
\noindent{\bf Discrete Transitions.}
A discrete transition $\transition=\tuple{\state_1,\state_2,\inputs,\reads,\outputs}$ 
in $\tpn$ is simulated by a set of transitions in $\sdtn$.
%
In defining this set, we take into consideration several aspects
of the simulation procedure as follows:
\begin{itemize}
\item
%
Basically, an interval $\interval$ 
on an arc leading from an input place $\place\in\inputs$ to
$\transition$   induces a set of transitions in $\transitions^\sdtn$; namely
transitions where there are arcs from places $\zeroplace{\place}{k}$ with $k\in\interval$, and
from places $\lowplace{\place}{k}$ and  $\highplace{\place}{k}$
with $(k+\epsilon)\in\interval$ for some
$\epsilon:0<\epsilon<1$.
%
An analogous construction is made for output and read places of $\transition$.
%
Since a read arc does not remove the token from the place, 
there is both an input arc and output arc to the corresponding transition in $\sdtn$.
%
\item
We recall that the tokens belonging to $\cmset_{-m'},\ldots,\cmset_{-1}$
are not generated during the initial phase, and that these tokens are gradually
introduced during the simulation phase.
%
Therefore, a transition may need to be fired before the 
required $\highplace{\place}{k}$-tokens have been produced by $\automaton$.
%
Such tokens are needed for performing both input and read operations.
%
In order to cover for tokens that are needed for input arcs, 
we use the set of places $\inputdebtplace{\place}{k}$
for $\place\in\places$ and $0\leq k\leq\maxval+1$.
%
Then, consuming a token from a place  $\highplace{\place}{k}$
may be replaced by putting a token in $\inputdebtplace{\place}{k}$.
%
The ``debt'' can be paid back using tokens 
that are later generated by $\automaton$.
%
When $\sdtn$ terminates, we require all the debt places to be empty
(all the debt has been paid back.)
%
Also, we need an analogous (but different) scheme for the 
read arcs.
%
The difference is due to the fact that
the same token may be read several times (without being consumed.)
%
Hence, once the debt has been introduced by the first read operation, it will not
be increased by the subsequent read operations.
%
Furthermore, several read operations may be covered by a (single)
input operation (a token in a place may be read several times before 
it is finally consumed through an input operations.)
%
To implement this, we use the variables $\rdebt{\place}{k}$.
%
Each time a number $r$ of tokens $\tuple{\place,k}$ are ``borrowed'' for a read operation,
we increase the value of $\rdebt{\place}{k}$ to $r$ (unless it already has a higher value.)
%
Furthermore, each debt taken on a token $\tuple{\place,k}$ in an input operation
subsumes a debt performed on the same token $\tuple{\place,k}$ in a read operation.
%
Therefore, the value of an old read debt is decreased by the amount
of the input debt taken during the current transition.
%
In a similar manner to input debts, the read debt
is later paid back.
%
When $\sdtn$ terminates, we require all $\rdebt{\place}{k}$
variables to be equal to $0$
(all the read debts have been paid back.)
%
\item
The transition also changes the control-state of $\tpn$.
%
\end{itemize} 







To formally define the set of transitions in $\sdtn$ induced by discrete transitions, 
we use a number of definitions.
%
We define $x\monus y:=\max(y-x,0)$.
%
For $k\in\nat$ and an interval $\interval$, we write
$k\inn\interval$ to denote that $(k+\epsilon)\in\interval$ for some (equivalently all) $\epsilon:0<\epsilon<1$.
%
During the simulation phase, there are two mechanisms for simulating
the effect of a token traveling through an (input, read, or output) arc in $\tpn$,
namely, (i)  by letting a token travel from (or to) a corresponding place;  and
(ii) by ``taking debt''.
 %
Therefore, we define a number of ``transformers'' that translate tokens 
in $\tpn$ to corresponding ones in $\sdtn$ as follows:
\begin{itemize}
\item
$\zeroplacetransform{\place,\interval}:=\setcomp{\zeroplace{\place}{k}}{(0\leq k\leq\maxval+1) \wedge(k\in\interval)}$.
%
The $\tpn$-token is simulated
by a $\sdtn$-token in a
place that represent tokens
with zero fractional parts.

\item
$\lowplacetransform{\place,\interval}:=\setcomp{\lowplace{\place}{k}}{(0\leq k\leq\maxval+1) \wedge (k\inn\interval)}$.
%
The $\tpn$-token is simulated
by a $\sdtn$-token in a
place that represent tokens
with low fractional parts.
%
Notice that we use the relation $\inn$ since the fractional part of the token is not zero.
\item
$\highplacetransform{\place,\interval}:=\setcomp{\highplace{\place}{k}}{(0\leq k\leq\maxval+1) \wedge (k\inn\interval)}$.
%
The $\tpn$-token is simulated
by a $\sdtn$-token in a
place that represent tokens
with high fractional parts.
%
\item
$\inputdebttransform{\place,\interval}:=\setcomp{\inputdebtplace{\place}{k}}{(0\leq k\leq\maxval+1) \wedge (k\inn\interval)}$. %
%
The $\tpn$-token is simulated by taking debt on an input token.
\item
$\readdebttransform{\place,\interval}:=\setcomp{\readdebtplace{\place}{k}}{(0\leq k\leq\maxval+1) \wedge (k\inn\interval)}$.
%
The $\tpn$-token is simulated by taking debt on a read token.
%
\end{itemize}
We extend the transformers to multisets,
so for a multiset $\mset=\lst{\tuple{\place_1,\interval_1},\ldots,\tuple{\place_{\ell},\interval_{\ell}}}$,
let 
$\zeroplacetransform{\mset}:=\!
\setcompdiv{\lst{\tuple{\place_1,k_1},\ldots,\tuple{\place_{\ell},k_{\ell}}}}
{\!\!\forall i:\!1\!\leq\! i\leq\ell:\tuple{\place_i,k_i}\!\in\!\!}{\zeroplacetransform{\place_i,\interval_i}}
$.
We extend the other definition to  multisets analogously.
%

An $\rdebtz$-mapping $\rdebtmapping$ is a function that maps each
$\rdebt{\place}{k}$ to a value in $\set{0,\ldots,\maxread}$.
%
In other words, the function describes the state of the debt on read
tokens.

Now, we are ready to define the transitions in $\sdtn$ that are
induced by discrete transitions in $\tpn$.
%
Each such a transition is induced by a number of objects, namely:
\begin{itemize}
\item
A transition $\transition = \tuple{\state_1,\state_2,\inputs,\reads,\outputs}\in\transitions$.
%
This is the transition in $\tpn$ that is to be simulated in $\sdtn$.
%
\item
The current remaining cost 
$y:\costof\transition\leq y\leq y_{\it init}$.
%
The remaining cost has to be at least as large as the
cost of the transition to be fired.
\item
An $\rdebtz$-mapping $\rdebtmapping$ describing the current debt on read tokens.
\item
Multisets 
$\inputs^{\it Zero},\inputs^{\it Low},\inputs^{\it High},\inputs^{\it Debt}$
where 
$\inputs=\inputs^{\it Zero}+\inputs^{\it Low}+\inputs^{\it High}+\inputs^{\it Debt}$.
%
Intuitively, the tokens traveling through arcs of $\transition$
are covered by fours types of tokens:
\begin{itemize}
\item
$\inputs^{\it Zero}$: $\tpn$-tokens that will be transformed
into $\sdtn$-tokens in places encoding ages with zero fractions parts.
\item
$\inputs^{\it Low}$: $\tpn$-tokens that will be transformed
into $\sdtn$-tokens in places encoding ages with low fractions parts.
\item
$\inputs^{\it High}$: $\tpn$-tokens that will be transformed
into $\sdtn$-tokens in places encoding ages with high fractions parts.
\item
$\inputs^{\it Debt}$: $\tpn$-tokens that will be covered by taking debt.
\end{itemize}
\item
Multisets $\reads^{\it Zero},\reads^{\it Low},\reads^{\it High},\reads^{\it Debt}$
where 
$\reads=\reads^{\it Zero}+\reads^{\it Low}+\reads^{\it High}+\reads^{\it Debt}$.
%
The roles of these multisets are similar to above.
\item
Multisets $\outputs^{\it Zero},\outputs^{\it Low},\outputs^{\it High}$
where 
$\outputs=\outputs^{\it Zero}+\outputs^{\it Low}+\outputs^{\it High}+\outputs^{\it Debt}$.
%
The roles of the multisets $\outputs^{\it Zero},\outputs^{\it Low},\outputs^{\it High}$
are similar to their counter-parts above.
%
\end{itemize}
For each such a collection of objects
(i.e., for each $\transition$, $0\leq y\leq y_{\it init}$, $\alpha$,
$\inputs^{\it Zero},\inputs^{\it Low},\inputs^{\it High},\inputs^{\it Debt}$,
$\reads^{\it Zero},\reads^{\it Low},\reads^{\it High},\reads^{\it Debt}$,
$\outputs^{\it Zero},\outputs^{\it Low},\outputs^{\it High}$),
we add the transition generator $\transgen$ where:
%
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\discmode,\nstate=\tuple{\state_1,y}}\cup\alpha$,
i.e., the current mode is $\discmode$, the current state of 
$\tpn$ is $\tuple{\state_1,y}$, and the current debt on read tokens is given
by $\alpha$.
\item
$\postcondof{\transgen}=\\
\set{\mode\assigned\simmode,\nstate\assigned\tuple{\state_2,y-\costof\transition}}\cup$\\
$\setcompdiv{\rdebt{\place}{k}
\assigned\max(\alpha\monus\inputs^{\it Debt'},\reads^{\it Debt'})(\place,k)}{}
{\!\!\!(\place\in\places)\wedge (0\!\leq\! k\!\leq\!\maxval\!+\!1)}$,
where 
\begin{itemize}
\item
$\inputs^{\it Debt'}=\inputdebttransform{\inputs^{\it Debt}}$.
\item
$\reads^{\it Debt'}=\readdebttransform{\reads^{\it Debt}}$.
\end{itemize}
%
In other words,
we change the mode back to $\simmode$, and change the control-state
of $\tpn$ to $\tuple{\state_2,y-\costof\transition}$.
%
The new read debts are defined as follows:
We reduce the current debt $\alpha$ 
using the new debt on input tokens $\inputs^{\it Debt'}$,
then we update the amount again using the new debt $\reads^{\it Debt'}$.
\item
$\inputsof{\transgen}=
\inputs^{\it Zero'}+\inputs^{\it Low'}+\inputs^{\it High'}+
\reads^{\it Zero'}+\reads^{\it Low'}+\reads^{\it High'}$, where
\begin{itemize}
\item
$\inputs^{\it Zero'}=\zeroplacetransform{\inputs^{\it Zero}}$.
\item
$\inputs^{\it Low'}=\lowplacetransform{\inputs^{\it Low}}$.
\item
$\inputs^{\it High'}=\highplacetransform{\inputs^{\it High}}$.
\item
$\reads^{\it Zero'}=\zeroplacetransform{\reads^{\it Zero}}$.
\item
$\reads^{\it Low'}=\lowplacetransform{\reads^{\it Low}}$.
\item
$\reads^{\it High'}=\highplacetransform{\reads^{\it High}}$.
%
\end{itemize}
The multisets 
$\inputs^{\it Zero},\inputs^{\it Low},\inputs^{\it High}$
represent tokens that will be consumed
due to input arcs.
%
These tokens are distributed among places according to 
whether their fractional parts are zero, low, or high.
%
A similar reasoning holds for the multisets
$\reads^{\it Zero},\reads^{\it Low},\reads^{\it High}$.
%
\item
$\outputsof{\transgen}=
\outputs^{\it Zero'}+\outputs^{\it Low'}+\outputs^{\it High'}+\outputs^{\it Debt'}+
\reads^{\it Zero'}+\reads^{\it Low'}+\reads^{\it High'}$, where
\begin{itemize}
\item
$\outputs^{\it Zero'}=\zeroplacetransform{\outputs^{\it Zero}}$.
\item
$\outputs^{\it Low'}=\lowplacetransform{\outputs^{\it Low}}$.
\item
$\outputs^{\it High'}=\highplacetransform{\outputs^{\it High}}$.
\item
$\outputs^{\it Debt'}=\highplacetransform{\inputs^{\it Debt}}$.
\item
$\reads^{\it Zero'}=\zeroplacetransform{\reads^{\it Zero}}$.
\item
$\reads^{\it Low'}=\lowplacetransform{\reads^{\it Low}}$.
\item
$\reads^{\it High'}=\highplacetransform{\reads^{\it High}}$.
%
\end{itemize}
%
The read multisets are defined in the previous item.

The multisets $\outputs^{\it Zero},\outputs^{\it Low},\outputs^{\it High}$ play the same roles
as their input and read counterparts.
%
The multiset $\outputs^{\it Debt'}$ represents the increase in the debt on 
read tokens.
\end{itemize}





\medskip
\noindent{\bf Transitions of Type $1$.}
%
The simulation of a type $1$ transition is started when the mode is
$\typeoneamode$.
%
We recall that a type $1$ transition encodes that time passes so that
all  tokens of integer age in $\mset_0$ will now have a positive fractional part,
but no tokens reach an integer age.
%
This phase is performed in two steps.
%
First, in $\typeoneamode$ (that is repeated an arbitrary number of times), 
some of these tokens are used for 
covering the multisets of $\finalmarking$
in a similar manner to the previous phases.
%
In the second step we
change mode to $\typeonebmode$, at the same time
switching $\on$ or $\off$ the component $\coverflag$
in a similar manner to the initialization phase.
%
In $\typeonebmode$, the (only set) of transfer transitions
encodes the effect of passing time.
%
%
More precisely all tokens in a 
place  $\zeroplace{\place}{k}$ will be moved to the place
$\lowplace{\place}{k}$, for $k:1\leq k\leq\maxval+1$.
%
From $\typeonebmode$ the mode will be changed
to $\typetwoamode$.
%

To describe $\typeoneamode$ formally we add,
for each $i:1\leq i\leq n$, $j:1\leq j\leq n_i$,
$\place\in\places$, $k:0\leq k\leq \maxval+1$
with $\tuple{\place,k}=\tuple{\place_{i,j},k_{i,j}}$,
a transition generator $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\typeoneamode,\coverflag=\on,\coverindex=i\}$.
\item
$\postcondof{\transgen}=\set{\fstate{i,j}\assigned\true}$.
\item
$\inputsof{\transgen}=\set{\zeroplace{\place}{k}}$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
%

On switching to $\typeonebmode$, we  change
the variables $\coverflag$ and $\coverindex$ in 
a similar manner to the previous phases.
%
Therefore, we add the following transition generators:

(i) 
For each $i:1\leq i\leq n$, and $i':-m\leq i'<i$,
we add $\transgen$ where:
%
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\typeoneamode,$ 
$\coverflag=\on,\coverindex=i\}$.
\item
$\postcondof{\transgen}=\{\mode\assigned\typeonebmode,\coverflag\assigned\off,\coverindex\assigned i'\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}

(ii) 
For each 
$i:1\leq i\leq n$, and $i':-m\leq i'<i$,
we add $\transgen$ where
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\typeoneamode,$ 
$\coverflag=\on,\coverindex=i\}$.
\item
$\postcondof{\transgen}=\{\mode\assigned\typeonebmode,$
$\coverindex\assigned i'\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}

(iii)
We add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\typeoneamode,$
$\coverflag=\off\}$.
\item
$\postcondof{\transgen}=\{\mode\assigned\typeonebmode\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}

(iv)
We add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\typeoneamode,$
$\coverflag=\off\}$.
\item
$\postcondof{\transgen}=\{\mode\assigned\typeonebmode,$
$\coverflag\assigned\on\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}


The set of transfer transitions is defined by the transfer
transition generator $\transgen$


\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\typeonebmode}$.
\item
$\postcondof{\transgen}=\set{\mode\assigned\typetwoamode}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\item
$\stof{\transgen}=\setcompdiv{\tuple{\zeroplace{\place}{k},\lowplace{\place}{k}}}{}
{(\place\in\places)\wedge(0\leq k\leq\maxval+1)}
$.
\end{itemize}


\medskip
\noindent{\bf Transitions of Type $2$.}
%
Recall that transitions of type $2$ 
encode what happens to tokens with the largest fractional parts
when an amount of time passes sufficient
for making these ages
equal to the next integer (but not larger.)
%
There are two sources of such tokens.
%
The generation of tokens according to these two sources 
divides the phase into two steps.
%
The first source are tokens that are currently in places
of the form $\highplace{\place}{k}$.
%
In $\typetwoamode$, (some of) these tokens reach the next integer, 
and are therefore moved to the corresponding
places encoding tokens with zero fractional parts.
%
As mentioned above,
only some (but not all) of these tokens reach the next integer.
%
The reason is that they are generated during the computation (not
by $\automaton$), and hence they have arbitrary fractional parts.


%
The second source are tokens that are provided by the automaton $\automaton$
(recall that these tokens are not generated during the initialization phase.)
%
In $\typetwobmode$, we run the automaton $\automaton$ one step at a time.
%
At each step we generate the next token
by taking a transition $\state_1\movesto{\tuple{\place,k}}\state_2$.
%
In fact, such a token $\tuple{\place,k}$ is used in two ways:
either it moves to the place $\zeroplace{\place}{k}$, or
it is used to pay the debt we have taken on tokens.
%
The debt is paid back either
(i) by removing
a token from $\inputdebtplace{\place}{k}$; or
(ii) by decrementing the value of the variable $\rdebt{\place}{k}$.
%
A transition $\state_1\movesto{\sep}\state_2$ means that we have 
read the last element of the current multiset.
%
This finishes simulating the transitions of type $1$ and $2$  and the mode is moved back
to $\simmode$ starting another iteration of the simulation phase.


Formally, we describe the movement of tokens in $\typetwoamode$
by adding,
for each $\place\in\places$ and $k:0\leq k\leq\maxval+1$, 
a transition generator $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\typetwoamode}$.
\item
$\postcondof{\transgen}=\emptyset$.
\item
$\inputsof{\transgen}=\set{\highplace{\place}{k}}$.
\item
$\outputsof{\transgen}=\set{\zeroplace{\place}{\max(k+1,\maxval+1)}}$.
\end{itemize}
%
At any time, we can change mode from $\typetwoamode$ to $\typetwobmode$:
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\typetwoamode}$.
\item
$\postcondof{\transgen}=\set{\mode\assigned\typetwobmode}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
%
We can also move back from $\typetwoamode$ to
$\simmode$ without letting the automaton generate any tokens:
%
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\typetwoamode}$.
\item
$\postcondof{\transgen}=\set{\mode\assigned\simmode}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
%
We simulate $\typetwobmode$ as follows.
%
To describe the movement of tokens places representing
tokens with zero fractional parts we add,
for each transition
$\state_1\movesto{\tuple{\place,k}}\state_2$ in $\automaton$,
a transition generator $\transgen$ where:
%
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\typetwobmode,\astate=\state_1}$.
\item
$\postcondof{\transgen}=\set{\astate\assigned\state_2}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\set{\zeroplace{\place}{k}}$.
\end{itemize}
%
To describe the payment of debts on input tokens we add,
for each transition
$\state_1\movesto{\tuple{\place,k}}\state_2$ in $\automaton$,
a transition generator $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\typetwobmode,\astate=\state_1}$.
\item
$\postcondof{\transgen}=\set{\astate\assigned\state_2}$.
\item
$\inputsof{\transgen}=\set{\inputdebtplace{\place}{k}}$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
%
To describe the payment of debts on read tokens we add,
for each transition
$\state_1\movesto{\tuple{\place,k}}\state_2$ in $\automaton$,
and $r:1\leq r\leq\maxread$,
a transition generator $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\typetwobmode,\astate=\state_1,\rdebt{\place}{k}=r}$.
\item
$\postcondof{\transgen}=\set{\astate\assigned\state_2,\rdebt{\place}{k}\assigned r-1}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
%



As usual, transition
$\state_1\movesto{\sep}\state_2$ in $\automaton$ indicates
means that we have 
read the last element of the current multiset.
%
We can now move back to the mode $\simmode$,
changing
the variables $\coverflag$ and $\coverindex$ in 
a similar manner to the previous phases.
%


(i)
For each transition of the form
$\state_1\movesto{\sep}\state_2$ in $\automaton$ ,
$i:1\leq i\leq n$, and $i':-m\leq i'<i$,
we add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\typetwobmode,\astate=\state_1,$ 
$\coverflag=\on,\coverindex=i\}$.
\item
$\postcondof{\transgen}=\{\mode\assigned\simmode,\astate\assigned\state_2,$
$\coverflag\assigned\off,\coverindex\assigned i'\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}

(ii)
For each transition $\state_1\movesto{\sep}\state_2$ in $\automaton$,
$i:1\leq i\leq n$, and $i':-m\leq i'<i$,
we add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\typetwobmode,\astate=\state_1,$ 
$\coverflag=\on,\coverindex=i\}$.
\item
$\postcondof{\transgen}=\{\mode\assigned\simmode,\astate\assigned\state_2,$
$\coverflag\assigned\on,\coverindex\assigned i'\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}

(iii)
For each transition
$\state_1\movesto{\sep}\state_2$ in $\automaton$,
we add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\typetwobmode,\astate=\state_1,$ 
$\coverflag=\off\}$.
\item
$\postcondof{\transgen}=\set{\mode\assigned\simmode,\astate\assigned\state_2}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}

(iv)
For each transition
$\state_1\movesto{\sep}\state_2$ in $\automaton$,
we add $\transgen$ where:

\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\typetwobmode,\astate=\state_1,$ 
$\coverflag=\off\}$.
\item
$\postcondof{\transgen}=\{\mode\assigned\simmode,\astate\assigned\state_2,$
$\coverflag\assigned\on\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
%




\medskip
\noindent{\bf The Final Phase.}
%
From the simulation mode we can at any time enter the final
mode.
%
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\simmode}$.
\item
$\postcondof{\transgen}=\set{\mode\assigned\finalonemode}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
%
The main tasks of the final phase are 
(i) to cover the multisets in $\finalmarking$;
and 
(ii) to continue paying back the \emph{debt} tokens (recall that the debt was partially
paid back in the simulation of type $2$ transitions.)
%
%
At the end of the final phase, we expect all tokens in $\finalmarking$ to have been
covered and all debt to have been paid back.
%
The final phase consists of two modes.
%
In $\finalonemode$ we cover the multisets in $\finalmarking$
using the tokens that have already been generated.
%
In $\finaltwomode$, we resume running $\automaton$ one step at a time.
%
The tokens generated from $\automaton$ are used both
(i) for paying back debt; and (ii) for covering the multisets 
$\mset_{-1},\ldots,\mset_{-m}$ (in that order.)
%


Formally, we add the following transition generators.
%
First, 
we continue covering the multisets $\mset_1,\ldots,\mset_n$.
%
For each $\place\in\places$, $1\leq i\leq n$, and $1\leq j\leq n_i$ with
$\tuple{\place_{i,j},k_{i,j}}=\tuple{\place,k}$, we add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\finalonemode}$.
\item
$\postcondof{\transgen}=\set{\fstate{i,j}\assigned\true}$.
\item
$\inputsof{\transgen}=\lowplace{\place}{k}$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
%
We cover the multiset $\mset_0$
by moving tokens from places of the form $\zeroplace{\place}{k}$.
%
For each $\place\in\places$ and $1\leq j\leq n_0$ with
$\tuple{\place_{0,j},k_{0,j}}=\tuple{\place,k}$, we add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\finalonemode}$.
\item
$\postcondof{\transgen}=\set{\fstate{0,j}\assigned\true}$.
\item
$\inputsof{\transgen}=\zeroplace{\place}{k}$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
%
We cover the multisets $\mset_{-1},\ldots,\mset_{-m}$
by moving tokens from places of the form $\highplace{\place}{k}$.
%
For each $\place\in\places$, $-m\leq i\leq -1$, $1\leq j\leq n_i$ with
$\tuple{\place_{i,j},k_{i,j}}=\tuple{\place,k}$, we add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\finalonemode}$.
\item
$\postcondof{\transgen}=\set{\fstate{i,j}\assigned\true}$.
\item
$\inputsof{\transgen}=\highplace{\place}{k}$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
We can change mode to $\finaltwomode$:
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\finalonemode}$.
\item
$\postcondof{\transgen}=\set{\mode\assigned\finaltwomode}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}

In $\finaltwomode$, we start running $\automaton$.
%
The tokens can be used for paying input debts.
%
For each transition
$\state_1\movesto{\tuple{\place,k}}\state_2$ in $\automaton$,
we add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\finaltwomode,\astate=\state_1}$.
\item
$\postcondof{\transgen}=\set{\astate\assigned\state_2}$.
\item
$\inputsof{\transgen}=\set{\inputdebtplace{\place}{k}}$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
%
The tokens can also be used for paying read debts.
%
For each transition
$\state_1\movesto{\tuple{\place,k}}\state_2$ in $\automaton$,
and $k:1\leq r\leq\maxread$,
we add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\set{\mode=\finaltwomode,\astate=\state_1,\rdebt{\place}{k}= r}$.
\item
$\postcondof{\transgen}=\set{\astate\assigned\state_2,\rdebt{\place}{k}\assigned r-1}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
%
Finally,
the tokens can  be used for covering.
%
For each transition
$\state_1\movesto{\tuple{\place,k}}\state_2$ in $\automaton$,
$i:-m\leq i\leq -1$, $j:1\leq j\leq n_i$,
$\place\in\places$, $k:0\leq k\leq \maxval+1$
with $\tuple{\place,k}=\tuple{\place_{i,j},k_{i,j}}$,
we have $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\finaltwomode,\coverflag=\on,\coverindex=i\}$.
\item
$\postcondof{\transgen}=\set{\fstate{i,j}\assigned\true}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
A transition
$\state_1\movesto{\sep}\state_2$ in $\automaton$ indicates
that we have 
read the last element of the current multiset.
%
We now let $\automaton$ generate the next multiset.
%
We change
the variables $\coverflag$ and $\coverindex$ in 
a similar manner to the previous phases.
%

(i)
For each transition of the form
$\state_1\movesto{\sep}\state_2$ in $\automaton$ ,
$i:-m\leq i\leq -1$, and $i':-m\leq i'<i$,
we add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\finaltwomode,\astate=\state_1,$ 
$\coverflag=\on,\coverindex=i\}$.
\item
$\postcondof{\transgen}=\{\astate\assigned\state_2,$
$\coverflag\assigned\off,\coverindex\assigned i'\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}

(ii)
For each transition $\state_1\movesto{\sep}\state_2$ in $\automaton$,
$i:1\leq i\leq n$, and $i':-m\leq i'<i$,
we add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\finaltwomode,\astate=\state_1,$ 
$\coverflag=\on,\coverindex=i\}$.
\item
$\postcondof{\transgen}=\{\astate\assigned\state_2,\coverindex\assigned i'\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}

(iii)
For each transition
$\state_1\movesto{\$}\state_2$ in $\automaton$,
we add $\transgen$ where:
\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\finaltwomode,\astate=\state_1,$ 
$\coverflag=\off\}$.
\item
$\postcondof{\transgen}=\{\astate\assigned\state_2\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}

(iv)
For each transition
$\state_1\movesto{\$}\state_2$ in $\automaton$,
we add $\transgen$ where:

\begin{itemize}
\item
$\precondof{\transgen}=\{\mode=\finaltwomode,\astate=\state_1,$ 
$\coverflag=\off\}$.
\item
$\postcondof{\transgen}=\{\astate\assigned\state_2,\coverflag\assigned\on\}$.
\item
$\inputsof{\transgen}=\emptyset$.
\item
$\outputsof{\transgen}=\emptyset$.
\end{itemize}
%


\medskip
\noindent{\bf The Set $\finalsdtnconfs$}
contains all configurations $\tuple{\finalstate^\sdtn,\finalmarking^\sdtn}$
satisfying the following conditions:
%
\begin{itemize}
\item
$\finalstate^\sdtn(\nstate)=\finalstate$.
%
The AC-PTPN is in its final control-state.
\item
$\finalstate^\sdtn(\fstate{i,j})=\true$ 
for all $i:-m\leq i\leq n$ and $1\leq j \leq n_i$.
%
We have covered all tokens in $\finalmarking$.
\item
$\finalstate^\sdtn(\rdebt{\place}{k})=0$
for all $\place\in\places$ and $k:0\leq k\leq\maxval+1$.
%
We have paid back all debts on read tokens.
\item
$\finalmarking(\inputdebtplace{\place}{k})=0$
for all $\place\in\places$ and $0\leq k\leq\maxval+1$.
%
We have paid back all debts on input tokens.
\end{itemize}

% We give an example of a concrete computation that give rise to the above abstract computation.


\end{proof}

